Text Entry for XR Trove (TEXT): Collecting and Analyzing Techniques for Text Input in XR

Text entry for extended reality (XR) is far from perfect, and a variety of text entry techniques (TETs) have been proposed to fit various contexts of use. However, comparing between TETs remains challenging due to the lack of a consolidated collection of techniques, and limited understanding of how interaction attributes of a technique (e.g., presence of visual feedback) impact user performance. To address these gaps, this paper examines the current landscape of XR TETs by creating a database of 176 different techniques. We analyze this database to highlight trends in the design of these techniques, the metrics used to evaluate them, and how various interaction attributes impact these metrics. We discuss implications for future techniques and present TEXT: Text Entry for XR Trove, an interactive online tool to navigate our database.

==> CodeBook.tex <==
% \usepackage{color}
% \usepackage{tabularray}
\definecolor{FrenchGray}{rgb}{0.749,0.749,0.752}
\begin{longtblr}[
  caption = {Codes and their Descriptions},
]{
  width = \linewidth,
  colspec = {Q[100]Q[105]Q[225]Q[550]},
  row{1} = {c},
  cell{2}{1} = {c,t},
  cell{7}{1} = {c,t},
  cell{20}{1} = {c,t},
  hline{2,7,20,34} = {-}{},
  hline{3-6,8-19,21-33} = {2-4}{FrenchGray},
}
\textbf{Category} & \textbf{Code} & \textbf{Description} & \textbf{Options (if applicable)}\\
\textbf{General } & \textbf{Source} & Where did the technique originate from? & {\textbf{Industry}: The technique's developement involved a person wokring at a company\\\textbf{Academia}: The technique's developement involved a person working at a university\\\textbf{Hobbyists}: The technique was developed by an individual on their own time}\\
 & \textbf{Date} & The date the technique was made public & \\
 & \textbf{Study} & Was a user study conducted? & {Yes \\No}\\
 & \textbf{Phrase Sets} & The phrase set used for evaluation & \\
 & \textbf{Other metrics} & Other metrics reported for evaluation beyond~speed, accuracy and NASA-TLX & \\
\textbf{Attributes} & \textbf{Input \\Device} & The hardware that is used to input the letters & {\textbf{None}: If the technique uses hand-tracking or eye-tracking built into commercial headsets and no other device\\\textbf{Controller}: If commercial VR controllers are used to enter the letters\\\textbf{Physical Keyboard}: If a keyboard is used to enter the letters\\\textbf{Touchscreen}: If a smartphone/tablet or a touch-sensitive surface is used\\\textbf{Custom hardware}: If any other device is used that doesn't come with a VR headset/controller}\\
 & \textbf{Body part (for input)} & The body part used for entering text & {\textbf{Finger(s)}: applies when users can directly enter text with their fingers(through hand tracking or touch sensing or some other technique)\\\textbf{Hand(s)}: When one or two hands are used to enter text. Cases that include using VR controllers fall under this category since the user holds and hovers over keys with their whole hand.\\\textbf{Gaze}: when text entry (or part of it) is done through gaze. If gaze can be used in combination with fingers and hands, enter both gaze and the other body part for input (fingers, hands)\\\textbf{Head}: when users hover over text with their head movement\\\textbf{Voice}: When text entry uses speech to text or voice commands}\\
 & \textbf{Concurrency} & How many pointers does the user have~in the virtual environment for text entry & {\textbf{One}: if one controller or gaze or a single finger is used.\\\textbf{Two}: If two controllers or fingers are used.\\\textbf{Multiple}: If more than two fingers are used. Ten-finger typing will fall under this category.}\\
 & \textbf{Haptic feedback modality} & Source of haptic feedback & {\textbf{None}: for mid-air typing with no haptic feedback\\\textbf{Button Press}: If the haptic feedback is from pressing a key on the controller/keyboard\\\textbf{External surface}: If any surface other the user body or custom hardware is used (e.g., a table or a board) to provide physical/force feedback for key presses. This code applies to typing with fingers.\\\textbf{On-body}: If the typing is done on the user body. The user body (e.g., arm, hands, legs, or other body parts) provides the physical support for key presses\\\textbf{Vibrotactile}: If a vibration is provided for hovering or key press. The vibration can be from controllers or from a custom haptic device.\\\textbf{Force feedback}: If a kinesthetic haptic device provides feedback on key hovering or key press.}\\
 & \textbf{Haptic feedback} & For what events or user actions~haptic feedback is provided to users & {\textbf{None}: No feedback is provided\\\textbf{Hovering}: Feedback is provided when a pointer is moved over a key before selection\\\textbf{Key Activation}: Feedback is provided after selection is confirmed}\\
 & \textbf{Audio feedback} & For what events or user actions~audio feedback is provided to users & {\textbf{None}: No feedback is provided\\\textbf{Hovering}: Feedback is provided when a pointer is moved over a key before selection\\\textbf{Key Activation}: Feedback is provided after selection is confirmed}\\
 & \textbf{Visual Feedback} & For what events or user actions~visual feedback is provided to users & {\textbf{None}: No feedback is provided\\\textbf{Hovering}: Feedback is provided when a pointer is moved over a key before selection\\\textbf{Key Activation}: Feedback is provided after selection is confirmed}\\
 & \textbf{Visual body representation} & How is the user presented visually & {\textbf{Invisible}: If no visual feedback is provided of the location of the user's input pointer (finger, hand, gaze)\\\textbf{Cursor/Pointer}: If one or two pointers (e.g., dots, crosses, pointer) are presented to show the key that is targeted\\\textbf{Controllers}: If the VR controllers are visible in VR\\\textbf{Fingertips}: If user's fingertips are in VR. This applies to cases where hand tracking is used\\\textbf{Bones}: If the skeleton of the user's hand(s) for one or more fingers are shown. This applies to cases where hand tracking is used.\\\textbf{Full hand}: If an avatar(s) of full hand(s) are shown in VR or if the real user hand can be seen (passthrough or AR).\\\textbf{Rays or drums}: When the pointer is connected to VR controller or the user hand with a ray or line.}\\
 & \textbf{Visual keyboard representation} & The way is the keyboard represented visually. & {\textbf{\textbf{None}}: If no keyboard is present. For example when handwriting or voice input is involved\textbf{}\\\textbf{Passthrough}: the user sees the physical keyboard or surface\\\textbf{Virtual overlay}: when there is a physical keyboard or surface but instead of seeing the actual keyboard or surface, a virtual keyboard is overlayed on it\\\textbf{Virtual }keyboard: There is no passthrough of the physical space and you only see virtual content/keyboard}\\
 & \textbf{Keyboard layout} & Order and layout of keys & \\
 & \textbf{Keyboard backend} & Algorithms that assist with the text entry~~by processing how typing is being performed & {\textbf{None}: if no algorithm is used to improve/assist in text entry\\\textbf{Prediction}: If words are predicted and suggested to users as user enters letters\\\textbf{Correction}: If typos (typing errors) are detected and corrections are suggested to users or applied directly\\\textbf{Personalization}: If the algorithm learns the users typing patterns (most frequency words, errors) and adjusts the suggestions or the keyboard layout or some other aspect to improve typing}\\
 & \textbf{Can be mobile?} & The mobility state of the user while entering text & {\textbf{Stationary}: If the technique can only be used when the user is not moving. i.e., if typing with this technique while walking will significantly impair user performance.\\\textbf{On the go}: If the technique ïs designed to enable" text entry on the go e.g., during walking or in transit. If there are specific design considerations for using the technique on the go. Of course, these techniques can also be used while stationary.}\\
 & \textbf{VR/AR} & For what XR technology was this technique developed & {\textbf{VR}: If the technique was only used/demonstrated in VR.\\\textbf{AR}: If the technique was only used/demonstrated in AR.\\\textbf{Both}: If the technique was used/demonstrated in both VR and AR.}\\
\textbf{Performance } & \textbf{WPM} & Typing speed in words per minute & \\
 & \textbf{CER} & Corrected error rate & \\
 & \textbf{UER} & Uncorrected error rate & \\
 & \textbf{TER} & Total error rate & \\
 & \textbf{MSD ER} & Minimum string difference error rate & \\
 & \textbf{ER} & Error rate & \\
 & \textbf{WER} & Word error rate & \\
 & \textbf{Overall TLX} & Overall score for NASA-TLX & \\
 & \textbf{Mental} & {The Mental subscale score of NASA-TLX} & \\
 & \textbf{Physical} & {The Physical subscale score of NASA-TLX} & \\
 & \textbf{Temporal} & {The Temporal subscale score of NASA-TLX} & \\
 & \textbf{Performance} & {The Performance subscale score of NASA-TLX} & \\
 & \textbf{Effort} & {The Effort subscale score of NASA-TLX} & \\
 & \textbf{Frustration} & {The Frustration subscale score of NASA-TLX} & 
\end{longtblr}
